A Vision Check-up for Language Models

What does learning to model relationships between strings teach large language models (LLMs) about the visual world? We systematically evaluate LLMs' abilities to generate and recognize an assortment of visual concepts of increasing complexity and then demonstrate how a preliminary visual representation learning system can be trained using models of text. As language models lack the ability to consume or output visual information as pixels, we use code to represent images in our study. Although LLM-generated images do not look like natural images, results on image generation and the ability of models to correct these generated images indicate that precise modeling of strings can teach language models about numerous aspects of the visual world. Furthermore, experiments on self-supervised visual representation learning, utilizing images generated with text models, highlight the potential to train vision models capable of making semantic assessments of natural images using just LLMs.

==> figures/cultural-bias/cultural-bias.tex <==
\begin{figure}[h]
    \centering
    \captionsetup[subfigure]{labelformat=empty,justification=centering,aboveskip=1pt,belowskip=1pt}
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \caption{English}        \includegraphics[width=0.98\linewidth,height=1.8cm]{figures/cultural-bias/a-flag_0.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \caption{Spanish}        
        \includegraphics[width=0.99\linewidth,height=2.8cm]{figures/cultural-bias/bandera_0.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \caption{Hindi}
        \includegraphics[width=0.99\linewidth,height=2.8cm]{figures/cultural-bias/झंडा_0.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \caption{Chinese}
        \includegraphics[width=0.99\linewidth,height=2.8cm]{figures/cultural-bias/旗帜_0.png}
    \end{subfigure}
    \par\smallskip
        \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=0.98\linewidth,height=2.8cm]{figures/cultural-bias/meal_0.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=0.99\linewidth,height=2.8cm]{figures/cultural-bias/alimento_0.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=0.99\linewidth,height=2.8cm]{figures/cultural-bias/खाना_0.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[trim= 50 120 50 0,clip,width=0.99\linewidth,height=2.8cm]{figures/cultural-bias/一顿饭_0.png}
    \end{subfigure}
    \caption{\textbf{The effect of language.} We ask the GPT-3.5 to draw a flag and a meal in four different languages. Surprisingly, the language used has a compelling effect on the generated content, hinting for cultural bias. This may hint that the model hold some visual cultural bias. %
}
    \label{fig:language}
\end{figure}


==> figures/retrival.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\linewidth]{figures/clip-percentile.pdf}
    \caption{\textbf{Image-text retrieval with clip-score.}}\label{fig:retrieval}
\end{figure}
